Transferring the driveshaft inertia to the grid via the DC-link in MV drive systems

This paper investigates a control approach that renders the driveshaft inertia completely available on the grid side and enhances the fault ride-through behavior of medium-voltage (MV) drive systems. Two main contributions are presented. First, we show how the rotational inertia of the driveline shaft can be synchronously coupled to the grid through a modification of the speed control reference signal and through an adapted DC-link control strategy. For the latter, we pursue two alternatives: one based on conventional cascaded control and another based on synchronous machine (SM) model matching. Second, we demonstrate that both the standard phase-locked loop (PLL) and the matching control approach can be interpreted, via the ray-circle complementarity, as feedback optimization schemes with distinct steady-state maps. This perspective allows us to revisit matching control, reveal its embedded PLL, highlight its current-limiting and tracking capabilities, and provide an extensive simulation study.

==> results_all.tex <==
%\newpage
\section{Experimental results}
\label{expRes}



Through a proprietary software-in-the-loop setup, we simulate a pumped-hydro drive system with a 7MVA grid-side transformer % whose grid impedance is show in Fig. \ref{Fig: Zgrid} 
and a 5kV DC-bus with mid-point. The converter is implemented using an average-model of the three-level active neutral-point-clamped (ANPC) topology. On the load-side, we implement a switching-model of the three-level ANPC converter connected to an Induction Machine (IM) model whose rotor is part of a 6MW driveline shaft modeled as a 5-mass torsional system as seen in Fig. \ref{Fig: dcmass}. 
The air-gap torque $\tau_m$ acts on one end of the shaft and the load $\tau_l$ on the other. 
%The motor torque is produced through a direct Model Predictive Control (MPC) which takes $\tau_m$ as reference, but 
%
The way in which the motor torque is produced (be it direct torque control, field-oriented control, or MPC) is not the focus of this work. 
%
For simplicity, we implement the projection $\Pi_\mathcal{C}$ via the activation-function approach in \cite{chandrasekaran2025reactive}.
%
For all our tests the speed reference is set to $w_\mathrm{nom}$ and we consider two grid scenarios: a stiff grid with an SCR of 49 and a weak grid with an SCR of 1. %, implying a 49 times larger impedance between the infinite bus source $v_\textit{grid}$ and the PCC. 

%\begin{remark}\label{obs2}
    We have used the cartesian implementation of the PLL with $\kappa_\textit{pll} = 63$, while the matching control structure uses $K_f = {7.54\mathsf{e\!-\!}3}$. For both approaches, we have used a virtual impedance $Z_v = 0.8 + J\omega_0{1\mathsf{e\!-\!}3}~\Omega$ while our model consisted of an impedance of $Z_g = {1\mathsf{e\!-\!}2} + J\omega_0{9\mathsf{e\!-\!}4}~\Omega$. The impedance between the PCC and the infinite bus was set to $Z_\textit{stiff} = {1.6\mathsf{e\!-\!}3} + J\omega_0{5.3\mathsf{e\!-\!}4}~\Omega$ in the stiff grid case, and to $Z_\textit{weak} = {8\mathsf{e\!-\!}2} + J\omega_0{2.58\mathsf{e\!-\!}3}~\Omega$, i.e. approx. $49$ times larger, in the weak grid case.
%\end{remark}


\subsection{Phase jump test}

We first set the load to $-0.5p.u.$, amounting to 2.93 MW of negative (generating) load. We compare side-by-side the response of the two control approaches to a 60-degree phase angle shift of the infinite bus $v_{grid}$. The stiff grid case is presented in Fig. \ref{Fig: strong_Angle} and the weak case in Fig. \ref{Fig: weak_Angle}.
%
\begin{figure*}[hb]
\centering{
\includegraphics[width=1\textwidth]{./figures/Tall_strong_angle22.pdf}
\caption{Grid angle phase shift of 60 degrees, stiff grid response. We see that both the PLL and the matching voltage respond in a well damped manner. However, the matching control voltage has a larger excursion than the cascaded PI's $v_{dc}$ which incurs a larger response from the coupling control on the mechanical side and excites the TNF, as seen in the inner-shaft torque $\tau_\textit{shaft}$.}	\label{Fig: strong_Angle}}
\end{figure*}
%
\begin{figure*}[hb]
\centering{
\includegraphics[width=1\textwidth]{./figures/Tall_weak_angle22.pdf}
\caption{Grid angle phase shift of 60 degrees, weak grid response. We see that the PLL has an underdamped response and cannot stabilize the AC voltage as well as the matching control, although it may be improved by tuning. This scenario shows the strength of the SM matching approach -- ride-through without reaching the current limit.}	\label{Fig: weak_Angle}}
\end{figure*}


\subsection{Three-phase drop test}

We then compare the response to a 5 second short-circuit of the infinite bus $v_{grid}$ at $-0.5p.u.$ mechanical load. The stiff and weak grid cases are presented in Fig. \ref{Fig: strong_Drop} and  \ref{Fig: weak_Drop}.
%
\begin{figure*}[hb]
\centering{
\includegraphics[width=1\textwidth]{./figures/Tall_strong_3drop.pdf}
\caption{Three-phase drop, stiff grid response. We see that the PCC drops to zero amplitude due to the low grid impedance. During this time the motor torque actually drops to zero preventing the DC-link to overcharge. This effect is simply the result of the elastic coupling that is enabled through the speed control and is beneficial. On the other hand, the reactive power is driven to zero due to the fact that the current magnitude saturates which forces the projection $\Pi_\mathcal{Q}$ to render zero reactive power demand. In fact, in the stiff grid situation the AC voltage regulator has very little effect throughout the tests.}	\label{Fig: strong_Drop}}
\end{figure*}
%
\begin{figure*}[hb]
\centering{
\includegraphics[width=1\textwidth]{./figures/Tall_weak_3drop.pdf}
\caption{Three-phase drop, weak grid response. Here we see that during the fault, the AC bus is sustained to the extent possible by a large capacitive current (negative $Q_g$) as a result of the AC voltage control \eqref{eq: qVC}. This feature is important for satisfying fault ride-through specifications found in e.g. IEC 61400. As before, $\tau_m$ drops to zero during the fault keeping the DC-link within limits. }	\label{Fig: weak_Drop}}
\end{figure*}


\subsection{Frequency step-up test}

Here we evaluate the response to a infinite bus $v_{grid}$ frequency step of $+1Hz$ again at $-0.5p.u.$. The stiff and weak grid cases are shown in Fig. \ref{Fig: strong_Fup} and \ref{Fig: weak_Fup}.
%
\begin{figure*}[hb]
\centering{
\includegraphics[width=1\textwidth]{./figures/Tall_strong_fup.pdf}
\caption{Grid frequency step up, stiff grid response. In this test the infinite bus frequency is well tracked by both the PLL and the electronic synchronous machine. What is remarkable is how the velocity of the driveshaft tracks the DC-link causing an active power response to the frequency change, just as intended. The difference between the two approaches is noticeable in the DC-link transient, the cascaded PI is subject to the bandwidth of the DC-link control \eqref{vdc_PI} while the matching approach has an instant response.}	\label{Fig: strong_Fup}}
\end{figure*}
%
\begin{figure*}[hb]
\centering{
\includegraphics[width=1\textwidth]{./figures/Tall_weak_fup.pdf}
\caption{Grid frequency step up, weak grid response. The difference here is mainly on the AC bus behavior, being more susceptible to disturbance and switching noise.}	\label{Fig: weak_Fup}}
\end{figure*}


\subsection{Single-phase drop test}

We now set the load to $0.95p.u.$, amounting to about 5.57 MW of positive (motoring) load. We now compare side-by-side the response of the two control approaches to a drop of one phase to zero. The stiff grid case is presented in Fig. \ref{Fig: strong_1ph} and the weak case in Fig. \ref{Fig: weak_1ph}.
%
\begin{figure*}[hb]
\centering{
\includegraphics[width=1\textwidth]{./figures/Tall_strong_1ph.pdf}
\caption{Single phase fault, stiff grid response. Due to the low impedance of the stiff grid the second harmonic of the line frequency affects the drive in similar ways for both approaches.}	\label{Fig: strong_1ph}}
\end{figure*}
%
\begin{figure*}[hb]
\centering{
\includegraphics[width=1\textwidth]{./figures/Tall_weak_1ph.pdf}
\caption{Single phase fault, weak grid scenario. We see that the matching control has an advantage over the cascaded PI in reducing the effect of the second harmonic.}	\label{Fig: weak_1ph}}
\end{figure*}


\subsection{Frequency step-down test}

With the load at $0.95p.u.$, we evaluate the response to a infinite bus $v_{grid}$ frequency step of $-1Hz$. The stiff and weak grid cases are presented in Fig. \ref{Fig: strong_Fdown} and \ref{Fig: weak_Fdown}. Note that in both frequency tests, a step of $1Hz$ is an extreme case and represents a change in drivetrain power of approx. $0.02p.u.$, a difference which is seen at the end of the transient.
%
\begin{figure*}[hb]
\centering{
\includegraphics[width=1\textwidth]{./figures/Tall_strong_fdown.pdf}
\caption{Grid frequency step down, stiff grid response. In this case we see a very similar performance between the two approaches and when compared to Fig. \ref{Fig: weak_Fup}.}	\label{Fig: strong_Fdown}}
\end{figure*}
%
\begin{figure*}[hb]
\centering{
\includegraphics[width=1\textwidth]{./figures/Tall_weak_fdown.pdf}
\caption{Grid frequency step down, weak grid. As in Fig. \ref{Fig: weak_Fup}, the difference is mainly on the AC bus behavior, being more susceptible to disturbance and switching noise.}	\label{Fig: weak_Fdown}}
\end{figure*}


\subsection{Voltage dip test}

We now perform the test in \cite{chandrasekaran2025reactive}, Section VA under similar conditions (again $0.95p.u.$ load). The stiff grid case is presented in Fig. \ref{Fig: strongDip} and the weak case in Fig. \ref{Fig: weak_Dip}.
%
\begin{figure*}[hb]
\centering{
\includegraphics[width=1\textwidth]{./figures/Tall_strong_3dip.pdf}
\caption{Voltage dip, stiff grid scenario. As a direct comparison to \cite{chandrasekaran2025reactive}, we see a similar behavior here where the current is well limited through the reactive power controller as well as the barrier function mechanism which implements the function of projection onto the constraint set.}	\label{Fig: strongDip}}
\end{figure*}
%
\begin{figure*}[hb]
\centering{
\includegraphics[width=1\textwidth]{./figures/Tall_weak_3dip.pdf}
\caption{Voltage dip, weak grid. We further note that the electronic synchronous machine behavior is different as the current tracking mechanism is different when compared to the cascaded PI. }	\label{Fig: weak_Dip}}
\end{figure*}


\subsection{Load reversal test}

Finally, we present a load step from $-0.5p.u.$ to $0.95p.u.$ under conditions of stiff grid in Fig. \ref{Fig: strongStep}, and weak grid in Fig. \ref{Fig: weak_Step}.
%
\begin{figure*}[hb]
\centering{
\includegraphics[width=1\textwidth]{./figures/Tall_strong_step.pdf}
\caption{Stiff grid, load step. The two control approaches yield similar results despite the difference in design philosophy.}	\label{Fig: strongStep}}
\end{figure*}
%
\begin{figure*}[hb]
\centering{
\includegraphics[width=1\textwidth]{./figures/Tall_weak_step.pdf}
\caption{Weak grid, load step. This test concludes the detailed comparison between the traditional cascade tracking approach and the novel, synchronous machine matching with energy-based control approach, yielding similar behavior. We see how the latter achieves current tracking, as well as modulation and current constraint satisfaction, in addition to the DC-link regulation, AC voltage support, and inertia provision features.}	\label{Fig: weak_Step}}
\end{figure*}
%
The complete set of experimental results can also be found on this git repository: {https://github.com/carghir/driveline-inertia-transfer/tree/v1.0}.





%\newpage





